Photometric Depth Super-Resolution

This study explores the use of photometric techniques (shape-from-shading and uncalibrated photometric stereo) for upsampling the low-resolution depth map from an RGB-D sensor to the higher resolution of the companion RGB image. A single-shot variational approach is first put forward, which is effective as long as the target's reflectance is piecewise-constant. It is then shown that this dependency upon a specific reflectance model can be relaxed by focusing on a specific class of objects (e.g., faces), and delegate reflectance estimation to a deep neural network. A multi-shot strategy based on randomly varying lighting conditions is eventually discussed. It requires no training or prior on the reflectance, yet this comes at the price of a dedicated acquisition setup. Both quantitative and qualitative evaluations illustrate the effectiveness of the proposed methods on synthetic and real-world scenarios.

==> tables/synthetic_comp_sfs_deep.tex <==
\begin{table*}[!ht]                                                                       
	\centering                                                                           
	\begin{tabular}{|c|c|c|cc|cc|cc|}                       
	
		\hline                                                                                                                          
		\multirow{2}{*}{Subject (S)}  & \multirow{2}{*}{Expression (E)}  & \multirow{2}{*}{SF} & \multicolumn{2}{c|}{\cite{Barron2015}} & \multicolumn{2}{c|}{\cite{Sfsnet18}} & \multicolumn{2}{c|}{Ours} \\\cline{4-9}
		&& & RMSE & MAE & RMSE & MAE & RMSE & MAE \\\hline                                                                                                                     
		\hline                                
	\multirow{30}{*}{11}& \multirow{2}{*}{0} & 2 & \textbf{0.1069} & 11.2811 & - & - & 0.1874 & \textbf{5.8277} \\            
%	\hline                                                                                                    
&	& 4 & 0.5148 & 41.7036 & 1.1023 & 12.2877 & \textbf{0.1217} & \textbf{7.0191} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{1} & 2 & \textbf{0.1110} & 12.1757 & - & - & 0.1774 & \textbf{5.9840} \\            
%	\hline                                                                                                    
&	& 4 & 0.6776 & 51.5362 & 1.2368 & 11.3087 & \textbf{0.1186} & \textbf{7.0827} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{2} & 2 & \textbf{0.1371} & 17.6559 & - & - & 0.1885 & \textbf{7.4410} \\            
%	\hline                                                                                                    
&	& 4 & 0.9092 & 58.2719 & 0.8175 & 19.8059 & \textbf{0.1463} & \textbf{9.7861} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{3} & 2 & \textbf{0.1200} & 13.1908 & - & - & 0.1935 & \textbf{6.2763} \\            
%	\hline                                                                                                    
&	& 4 & 0.7650 & 53.3137 & 1.2194 & 13.6341 & \textbf{0.1308} & \textbf{7.6617} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{4} & 2 & \textbf{0.1106} & 12.0300 & - & - & 0.1909 & \textbf{6.7654} \\            
%	\hline                                                                                                    
&	& 4 & 0.5584 & 49.2738 & 0.9065 & 13.1894 & \textbf{0.1354} & \textbf{8.0273} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{5} & 2 & \textbf{0.1964} & 14.5500 & - & - & 0.2068 & \textbf{7.3362} \\            
%	\hline                                                                                                    
&	& 4 & 0.6844 & 53.0044 & 1.0657 & 15.0912 & \textbf{0.1909} & \textbf{8.9047} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{6} & 2 & \textbf{0.1206} & 13.2598 & - & - & 0.1883 & \textbf{6.8373} \\            
%	\hline                                                                                                    
&	& 4 & 0.7318 & 57.4497 & 0.7211 & 14.3706 & \textbf{0.1398} & \textbf{8.3742} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{7} & 2 & 0.3674 & 15.1031 & - & - & \textbf{0.2287} & \textbf{7.2632} \\            
%	\hline                                                                                                    
&	& 4 & 0.6998 & 47.2498 & 1.0601 & 18.9270 & \textbf{0.2642} & \textbf{9.7440} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{8} & 2 & \textbf{0.1094} & 15.9824 & - & - & 0.1813 & \textbf{9.3954} \\            
%	\hline                                                                                                    
&	& 4 & 0.5888 & 55.8985 & 0.8822 & 13.4861 & \textbf{0.1147} & \textbf{9.8121} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{9} & 2 & \textbf{0.1118} & 12.3690 & - & - & 0.1714 & \textbf{6.7411} \\            
%	\hline                                                                                                    
&	& 4 & 0.5300 & 47.9372 & 0.9714 & 13.0998 & \textbf{0.1267} & \textbf{7.8888} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{10} & 2 & \textbf{0.1225} & 14.4960 & - & - & 0.1955 & \textbf{7.9537} \\           
%	\hline                                                                                                    
&	& 4 & 1.0062 & 55.9198 & 0.8631 & 17.9839 & \textbf{0.1417} & \textbf{8.9901} \\
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{11} & 2 & \textbf{0.1159} & 12.4566 & - & - & 0.1890 & \textbf{6.6804} \\           
%	\hline                                                                                                    
&	& 4 & 0.6296 & 49.2944 & 1.0929 & 12.4240 & \textbf{0.1563} & \textbf{7.7767} \\
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{12} & 2 & \textbf{0.1092} & 11.8244 & - & - & 0.1886 & \textbf{6.0235} \\           
%	\hline                                                                                                    
&	& 4 & 0.7968 & 51.1406 & 0.8824 & 11.0540 & \textbf{0.1207} & \textbf{7.2522} \\
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{13} & 2 & \textbf{0.1113} & 12.4305 & - & - & 0.1870 & \textbf{6.1529} \\           
%	\hline                                                                                                    
&	& 4 & 0.7014 & 52.5077 & 0.5021 & 10.0072 & \textbf{0.1322} & \textbf{7.3263} \\
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{14} & 2 & \textbf{0.1091} & 11.9522 & - & - & 0.1828 & \textbf{6.2014} \\           
%	\hline                                                                                                    
&	& 4 & 0.6463 & 49.8636 & 0.7394 & 11.3868 & \textbf{0.1212} & \textbf{7.3132} \\
	\hline                                                                                                    
	\multirow{30}{*}{4}& \multirow{2}{*}{0} & 2 & 0.2281 & 23.4415 & - & - & \textbf{0.1908} & \textbf{5.9752} \\             
%	\hline                                                                                                    
&	& 4 & 0.6488 & 49.1959 & 0.4741 & 13.9368 & \textbf{0.1117} & \textbf{6.8132} \\  
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{1} & 2 & 0.2854 & 30.5486 & - & - & \textbf{0.1849} & \textbf{6.9702} \\             
%	\hline                                                                                                    
&	& 4 & 0.5953 & 47.9548 & 1.0130 & 14.7240 & \textbf{0.1127} & \textbf{7.6400} \\  
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{2} & 2 & 0.2528 & 29.8795 & - & - & \textbf{0.1776} & \textbf{8.2012} \\             
%	\hline                                                                                                    
&	& 4 & 0.6011 & 55.0417 & 1.0439 & 18.9314 & \textbf{0.1284} & \textbf{9.7949} \\  
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{3} & 2 & \textbf{0.1888} & 19.0886 & - & - & 0.1927 & \textbf{7.7149} \\             
%	\hline                                                                                                    
&	& 4 & 0.6380 & 51.7959 & 0.6933 & 16.3201 & \textbf{0.1223} & \textbf{8.9794} \\  
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{4} & 2 & 0.2837 & 30.3095 & - & - & \textbf{0.1817} & \textbf{7.4706} \\             
%	\hline                                                                                                    
&	& 4 & 0.5122 & 45.8693 & 0.5258 & 15.4585 & \textbf{0.1138} & \textbf{8.5289} \\  
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{}5 & 2 & 0.3609 & 35.5668 & - & - & \textbf{0.2028} & \textbf{9.1059} \\             
%	\hline                                                                                                    
&	& 4 & 0.6447 & 54.1181 & 0.9701 & 19.2865 & \textbf{0.1970} & \textbf{11.2153} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{6} & 2 & 0.2205 & 27.0965 & - & - & \textbf{0.1995} & \textbf{8.0220} \\             
%	\hline                                                                                                    
&	& 4 & 0.5927 & 51.2974 & 1.0100 & 19.4058 & \textbf{0.1542} & \textbf{9.6648} \\  
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{7} & 2 & 0.2369 & 24.9252 & - & - & \textbf{0.2087} & \textbf{8.6590} \\             
%	\hline                                                                                                    
&	& 4 & 0.6050 & 49.9729 & 0.8597 & 20.1422 & \textbf{0.1941} & \textbf{9.5206} \\  
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{8} & 2 & 0.2145 & 26.4886 & - & - & \textbf{0.1827} & \textbf{8.0033} \\             
%	\hline                                                                                                    
&	& 4 & 0.5710 & 53.4401 & 0.7588 & 14.0183 & \textbf{0.1075} & \textbf{8.2670} \\  
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{9} & 2 & \textbf{0.1859} & 22.4924 & - & - & 0.1892 & \textbf{7.2511} \\             
%	\hline                                                                                                    
&	& 4 & 0.5734 & 50.5616 & 0.5135 & 14.7545 & \textbf{0.1169} & \textbf{8.5230} \\  
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{10} & 2 & 0.2744 & 28.8505 & - & - & \textbf{0.1877} & \textbf{7.0955} \\            
%	\hline                                                                                                    
&	& 4 & 0.6009 & 53.1664 & 0.5744 & 17.2112 & \textbf{0.1117} & \textbf{7.7747} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{11} & 2 & \textbf{0.1044} & 12.7931 & - & - & 0.1961 & \textbf{7.1938} \\            
%	\hline                                                                                                    
&	& 4 & 0.6136 & 52.9554 & 1.0092 & 14.1251 & \textbf{0.1115} & \textbf{7.6181} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{12} & 2 & \textbf{0.1814} & 21.9536 & - & - & 0.2034 & \textbf{6.8525} \\            
%	\hline                                                                                                    
&	& 4 & 0.6190 & 50.8171 & 0.6188 & 14.5414 & \textbf{0.1293} & \textbf{7.7816} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{13} & 2 & \textbf{0.1151} & 13.6560 & - & - & 0.1866 & \textbf{6.6517} \\            
%	\hline                                                                                                    
&	& 4 & 0.5817 & 51.1208 & 1.1871 & 14.8568 & \textbf{0.1115} & \textbf{7.7797} \\ 
	\cline{2-9}                                                                                                    
	& \multirow{2}{*}{14} & 2 & \textbf{0.1810} & 21.5087 & - & - & 0.1906 & \textbf{6.8284} \\            
%	\hline                                                                                                    
&	& 4 & 0.5812 & 49.7192 & 0.7939 & 14.3981 & \textbf{0.1111} & \textbf{7.6929} \\ 
	\hline
	\hline                                                   
%	\multicolumn{2}{|c|}{$\sum$} &  & 20 & 0 & 0 & 0 & 10 & 30 \\                                                                                                                                                                                                                                      
%	\hline                                                                                                       
	\multicolumn{2}{|c|}{\multirow{2}{*}{Median}} & 2 & 0.1590 & 15.5428 & - & - & 0.1888 & 7.0328 \\                                                
%	\hline                                                                                                    
	\multicolumn{2}{|c|}{}& 4 & 0.6163 & 51.2190 & 0.8823 & 14.4698 & 0.1245 & 7.9581 \\                                     
	\hline                                                                                                    
	\multicolumn{2}{|c|}{\multirow{2}{*}{Mean}}& 2 & 0.1791 & 18.9786 & - & - & 0.1911 & 7.1625 \\                                                  
%	\hline                                                                                                    
	\multicolumn{2}{|c|}{}& 4 & 0.6473 & 51.3797 & 0.8703 & 15.0056 & 0.1365 & 8.3518 \\ 
		\hline                                                                      
	\end{tabular}                                                                        
	\caption{Quantitative comparison between our method combining variational methods with machine learning, and two other state-of-the-art methods on two subjects from 3DRFE Dataset\cite{Database3drfe2007}. %Prior weights of SIRFS \cite{Barron2015} were tuned for better results. RMSE values for Pix2Vertex \cite{Pix2Vertex2017} are calculated by first computing the depth from the provided normals.
	}  
	\label{tab:deepnetTable}                                                                
\end{table*}  


==> tables/table_diligent_sfs.tex <==
\begin{table*}                                                                                                     
\centering                                                                                                         
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}                                                                             
\hline                                                                                                             
\multirow{2}{*}{3D-shape} & \multirow{2}{*}{SF} & \multicolumn{2}{c|}{\cite{Yang2007}}& \multicolumn{2}{c|}{\cite{Xie2016}}  & \multicolumn{2}{c|}{\cite{Or-El2015}}  & \multicolumn{2}{c|}{Ours}  \\                          
\cline{3-10}                                                                                                             
 &  & RMSE & MAE & RMSE & MAE & RMSE & MAE & RMSE & MAE \\                                                         
\hline                                                                                                             
\hline                                                                                                             
 & 2 & 1.155 & 14.6872 & -- & -- & 1.4501 & 10.4079 & \textbf{0.70552} & \textbf{8.384} \\                         
bear & 4 & \textbf{1.2327} & 17.9733 & 151.3218 & 31.3593 & 2.6627 & 15.1408 & 1.4249 & \textbf{11.428} \\         
 & 8 & 72.1766 & 66.3692 & -- & -- & 4.3978 & 18.5369 & \textbf{2.8456} & \textbf{18.022} \\                       
\hline                                                                                                             
 & 2 & 1.5449 & 28.1155 & -- & -- & 2.0532 & 26.8927 & \textbf{1.3398} & \textbf{24.1622} \\                       
buddha & 4 & \textbf{1.6272} & 29.9718 & 144.8857 & 36.2772 & 2.9809 & 29.4112 & 2.018 & \textbf{26.8779} \\       
 & 8 & 311.517 & 81.2595 & -- & -- & 4.0834 & \textbf{28.9055} & \textbf{3.3358} & 31.236 \\                       
\hline                                                                                                             
 & 2 & 1.4793 & 16.0352 & -- & -- & 1.5784 & \textbf{12.1009} & \textbf{1.3628} & 12.3755 \\                       
cat & 4 & \textbf{1.6517} & 20.2194 & 139.4621 & 31.719 & 2.6211 & 16.5566 & 2.1678 & \textbf{15.6201} \\          
 & 8 & \textbf{2.2937} & 24.5675 & -- & -- & 4.2572 & \textbf{19.6851} & 3.8145 & 22.5541 \\                       
\hline                                                                                                             
 & 2 & 1.2888 & 19.2754 & -- & -- & 1.3917 & \textbf{10.0119} & \textbf{0.84839} & 16.0584 \\                      
cow & 4 & \textbf{1.418} & 20.8781 & 146.8426 & 33.457 & 2.5341 & \textbf{12.872} & 1.542 & 16.4131 \\             
 & 8 & \textbf{1.9094} & 27.1148 & -- & -- & 4.5013 & \textbf{16.8404} & 3.1524 & 19.1884 \\                       
\hline                                                                                                             
 & 2 & 1.768 & 22.614 & -- & -- & \textbf{1.7428} & 12.1403 & 1.8322 & \textbf{11.9935} \\                         
goblet & 4 & \textbf{1.874} & 23.5636 & 224.0792 & 34.0678 & 2.8078 & 16.0514 & 2.8481 & \textbf{15.769} \\        
 & 8 & \textbf{2.5408} & 28.1004 & -- & -- & 3.711 & \textbf{16.7966} & 5.2276 & 20.791 \\                         
\hline                                                                                                             
 & 2 & 2.6586 & 27.1733 & -- & -- & \textbf{2.4706} & \textbf{23.0364} & 2.6945 & 24.6588 \\                       
harvest & 4 & 40094.1042 & 107.1357 & 128.8568 & 36.7433 & \textbf{3.8501} & \textbf{25.8813} & 3.9467 & 27.3619 \\
 & 8 & 530.889 & 88.9888 & -- & -- & 6.3268 & \textbf{27.037} & \textbf{6.2881} & 32.4737 \\                       
\hline                                                                                                             
 & 2 & 1.5155 & 19.2552 & -- & -- & 1.7272 & 12.6853 & \textbf{1.0772} & \textbf{11.4061} \\                       
pot1 & 4 & \textbf{1.5842} & 20.791 & 120.3992 & 32.1144 & 2.6075 & 15.1411 & 1.7001 & \textbf{13.6763} \\         
 & 8 & \textbf{2.2184} & 24.6515 & -- & -- & 3.585 & 17.9752 & 2.8789 & \textbf{16.7584} \\                        
\hline                                                                                                             
 & 2 & 1.5301 & 21.0721 & -- & -- & 1.4754 & 13.2556 & \textbf{0.85548} & \textbf{13.0964} \\                      
pot2 & 4 & 1.5286 & 22.0212 & 153.9197 & 33.052 & 2.6759 & 16.3269 & \textbf{1.4413} & \textbf{14.9414} \\         
 & 8 & \textbf{2.1033} & 27.3341 & -- & -- & 3.7331 & \textbf{18.0233} & 2.5797 & 19.4412 \\                       
\hline                                                                                                             
 & 2 & 2.03 & 24.6931 & -- & -- & 2.1182 & 17.008 & \textbf{1.626} & \textbf{14.2358} \\                           
reading & 4 & \textbf{2.0959} & 26.7387 & 156.7157 & 31.9848 & 3.6016 & 22.081 & 2.6705 & \textbf{19.9202} \\      
 & 8 & \textbf{2.9265} & 31.5624 & -- & -- & 5.5075 & \textbf{24.3578} & 5.0134 & 27.2754 \\                       
\hline                                                                                                             
\hline                                                                                                             
 & 2 & 1.5301 & 21.0721 & -- & -- & 1.7272 & \textbf{12.6853} & \textbf{1.3398} & 13.0964 \\                       
Median & 4 & \textbf{1.6272} & 22.0212 & 146.8426 & 33.052 & 2.6759 & 16.3269 & 2.018 & \textbf{15.769} \\         
 & 8 & \textbf{2.5408} & 28.1004 & -- & -- & 4.2572 & \textbf{18.5369} & 3.3358 & 20.791 \\                        
\hline                                                                                                             
 & 2 & 1.6634 & 21.4357 & -- & -- & 1.7786 & 15.2821 & \textbf{1.3713} & \textbf{15.1523} \\                       
Mean & 4 & 4456.3463 & 32.1436 & 151.8314 & 33.4194 & 2.9269 & 18.8291 & \textbf{2.1955} & \textbf{18.0009} \\     
 & 8 & 103.175 & 44.4387 & -- & -- & 4.4559 & \textbf{20.9064} & \textbf{3.904} & 23.0822 \\                       
\hline                                                                                                             
\end{tabular}                                                                                                      
\caption{Quantitative Comparison between other sota methods and our on DiliGenT data}                              
\label{table:tab:diligent_comparison_sfs}                                                                          
\end{table*}                                                                                                       


==> tables/table_diligent_sfs_deep.tex <==
\begin{table*}                                                                           
\centering                                                                               
\begin{tabular}{|c|c|c|c|c|c|c|c|}                                                       
\hline                                                                                   
		\multirow{2}{*}{3D-Shape}  & \multirow{2}{*}{SF} & \multicolumn{2}{c|}{\cite{Barron2015}} & \multicolumn{2}{c|}{\cite{Sfsnet18}} & \multicolumn{2}{c|}{Ours} \\\cline{3-8}
		& & RMSE & MAE & RMSE & MAE & RMSE & MAE \\\hline\hline                                
\multirow{2}{*}{bear} & 2 & 26.1695 & 131.2633 & -- & -- & \textbf{0.0044875} & \textbf{10.7725} \\       
                                                                                 
 & 4 & 17.5327 & 132.3312 & 0.045108 & 50.2167 & \textbf{0.0086406} & \textbf{15.1351} \\
\hline                                                                                   
\multirow{2}{*}{buddha} & 2 & 45.6078 & 106.5397 & -- & -- & \textbf{0.0083201} & \textbf{28.4893} \\     
 & 4 & 24.5214 & 110.6067 & 0.046625 & 47.2658 & \textbf{0.011993} & \textbf{32.1496} \\ 
\hline                                                                                   
\multirow{2}{*}{cat} & 2 & 44.2582 & 112.6649 & -- & -- & \textbf{0.0083353} & \textbf{13.384} \\         
 & 4 & 23.6849 & 119.1405 & 0.041393 & 44.1362 & \textbf{0.013241} & \textbf{16.4899} \\ 
\hline                                                                                   
\multirow{2}{*}{cow} & 2 & 20.6986 & 103.0394 & -- & -- & \textbf{0.0049759} & \textbf{14.4648} \\        
 & 4 & 18.0335 & 114.1518 & 0.033876 & 42.3159 & \textbf{0.009261} & \textbf{16.0579} \\ 
\hline                                                                                   
\multirow{2}{*}{goblet} & 2 & 58.2059 & 84.8205 & -- & -- & \textbf{0.011337} & \textbf{24.1657} \\       
 & 4 & 56.5 & 105.4519 & 0.10413 & 43.6249 & \textbf{0.01711} & \textbf{25.1141} \\      
\hline                                                                                   
\multirow{2}{*}{harvest} & 2 & 29.4218 & 100.4635 & -- & -- & \textbf{0.016384} & \textbf{36.6518} \\     
 & 4 & 22.9276 & 106.5154 & 0.079867 & 54.1843 & \textbf{0.023768} & \textbf{36.1969} \\ 
\hline                                                                                   
\multirow{2}{*}{pot1} & 2 & 8.8311 & \textbf{0} & -- & -- & \textbf{0.0071345} & 15.0327 \\               
 & 4 & 27.0375 & 117.929 & 0.059287 & 51.4572 & \textbf{0.010606} & \textbf{15.9852} \\  
\hline                                                                                   
\multirow{2}{*}{pot2} & 2 & 43.7269 & 97.1625 & -- & -- & \textbf{0.0056094} & \textbf{17.7692} \\        
 & 4 & 14.4535 & 108.8758 & 0.031794 & 41.3383 & \textbf{0.008765} & \textbf{18.3856} \\ 
\hline                                                                                   
\multirow{2}{*}{reading} & 2 & 8.8314 & \textbf{0} & -- & -- & \textbf{0.0098971} & 20.6394 \\            
 & 4 & 19.4357 & 107.2029 & 0.09295 & 56.2257 & \textbf{0.015739} & \textbf{23.1794} \\  
\hline\hline                                                                                   
Median & 2 & 29.4218 & 100.4635 & -- & -- & \textbf{0.0083201} & \textbf{17.7692} \\     
 & 4 & 22.9276 & 110.6067 & 0.046625 & 47.2658 & \textbf{0.011993} & \textbf{18.3856} \\ 
\hline                                                                                   
Mean & 2 & 31.7501 & 81.7726 & -- & -- & \textbf{0.0084978} & \textbf{20.1521} \\        
 & 4 & 24.903 & 113.5784 & 0.059448 & 47.8628 & \textbf{0.013236} & \textbf{22.0771} \\  
\hline                                                                                   
\end{tabular}                                                                            
\caption{Quantitative Comparison between other sota methods and our on DiliGenT data}    
\label{table:tab:diligent_comparison_sfs_deep}                                           
\end{table*}                                                                             


==> tables/table_diligent_sfs_joy_mag.tex <==
\begin{table*}                                                                                                    
\centering                                                                                                        
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}                                                                            
\hline                                                                                                            
\multirow{2}{*}{3D-shape} & \multirow{2}{*}{SF} & \multicolumn{2}{c|}{\cite{Yang2007}}& \multicolumn{2}{c|}{\cite{Xie2016}}  & \multicolumn{2}{c|}{\cite{Or-El2015}}  & \multicolumn{2}{c|}{Ours}  \\                          
\cline{3-10}                                                                                                             
 &  & RMSE & MAE & RMSE & MAE & RMSE & MAE & RMSE & MAE \\                                                        
\hline                                                                                                            
\hline                                                                                                            
 & 2 & 0.0067319 & 15.0387 & -- & -- & 0.059551 & 47.4345 & \textbf{0.0045354} & \textbf{11.7715} \\              
bear & 4 & \textbf{0.0071752} & 17.6883 & 0.90094 & 31.1833 & 0.056456 & 47.0729 & 0.0084408 & \textbf{13.5733} \\
 & 8 & 0.78277 & 74.7426 & -- & -- & 0.098455 & 45.3945 & \textbf{0.016887} & \textbf{20.849} \\                  
\hline                                                                                                            
 & 2 & 0.0092639 & 28.4836 & -- & -- & 0.094695 & 75.606 & \textbf{0.0081395} & \textbf{26.7243} \\               
buddha & 4 & \textbf{0.0093799} & 30.9444 & 0.83224 & 36.4599 & 0.13083 & 91.994 & 0.012 & \textbf{26.8097} \\    
 & 8 & 0.060714 & 38.3252 & -- & -- & 0.11055 & 62.06 & \textbf{0.020032} & \textbf{31.8447} \\                   
\hline                                                                                                            
 & 2 & 0.0087748 & 16.1544 & -- & -- & 0.067433 & 53.7429 & \textbf{0.0081252} & \textbf{14.4117} \\              
cat & 4 & \textbf{0.0099602} & 20.9329 & 0.79582 & 31.0152 & 0.085995 & 53.9512 & 0.0126 & \textbf{16.6402} \\    
 & 8 & 0.79402 & 56.4294 & -- & -- & 0.090679 & 48.9718 & \textbf{0.022035} & \textbf{22.5226} \\                 
\hline                                                                                                            
 & 2 & 0.0076319 & 19.4369 & -- & -- & 0.090132 & 58.421 & \textbf{0.0048842} & \textbf{15.2397} \\               
cow & 4 & \textbf{0.0081414} & 21.4438 & 0.84181 & 33.1486 & 0.083994 & 56.3389 & 0.0091083 & \textbf{15.8243} \\ 
 & 8 & \textbf{0.011573} & 25.8188 & -- & -- & 0.049626 & 25.5055 & 0.018031 & \textbf{18.6177} \\                
\hline                                                                                                            
 & 2 & \textbf{0.01083} & 22.5984 & -- & -- & 0.16494 & 76.2777 & 0.010861 & \textbf{13.6735} \\                  
goblet & 4 & \textbf{0.011623} & 25.0196 & 1.3301 & 34.2957 & 0.16403 & 77.9689 & 0.01671 & \textbf{15.1966} \\   
 & 8 & \textbf{0.015739} & 28.4787 & -- & -- & 0.14513 & 67.9802 & 0.031552 & \textbf{20.9878} \\                 
\hline                                                                                                            
 & 2 & \textbf{0.015663} & 27.3319 & -- & -- & 0.12607 & 72.0992 & 0.015724 & \textbf{23.0309} \\                 
harvest & 4 & 0.51134 & 47.1777 & 0.7631 & 36.4439 & 0.11961 & 71.1135 & \textbf{0.023277} & \textbf{27.6302} \\  
 & 8 & 193.2953 & 82.4501 & -- & -- & 0.12862 & 67.8287 & \textbf{0.037184} & \textbf{32.6538} \\                 
\hline                                                                                                            
 & 2 & 0.0092171 & 19.1262 & -- & -- & 0.024007 & 39.854 & \textbf{0.0060987} & \textbf{16.7937} \\               
pot1 & 4 & \textbf{0.0091357} & 20.8363 & 0.71928 & 31.9851 & 0.03327 & 29.1709 & 0.0096464 & \textbf{17.0921} \\ 
 & 8 & \textbf{0.013381} & 25.3591 & -- & -- & 0.064352 & 32.5091 & 0.015912 & \textbf{19.8503} \\                
\hline                                                                                                            
 & 2 & 0.0078003 & 18.7368 & -- & -- & 0.015572 & 31.5673 & \textbf{0.005009} & \textbf{16.3235} \\               
pot2 & 4 & 0.0086183 & 22.1641 & 0.8869 & 32.7756 & 0.039953 & 45.87 & \textbf{0.0078853} & \textbf{17.5155} \\   
 & 8 & \textbf{0.011221} & 26.5275 & -- & -- & 0.059238 & 44.5195 & 0.014543 & \textbf{19.147} \\                 
\hline                                                                                                            
 & 2 & 0.011917 & 25.5409 & -- & -- & 0.13391 & 64.7135 & \textbf{0.0096912} & \textbf{14.723} \\                 
reading & 4 & \textbf{0.012162} & 27.0008 & 0.91973 & 31.9683 & 0.13662 & 61.2494 & 0.015663 & \textbf{19.9486} \\
 & 8 & \textbf{0.015772} & 29.7582 & -- & -- & 0.1917 & 64.7146 & 0.029041 & \textbf{26.8748} \\                  
\hline                                                                                                            
\hline                                                                                                            
 & 2 & 0.0092171 & 19.4369 & -- & -- & 0.090132 & 58.421 & \textbf{0.0081252} & \textbf{15.2397} \\               
Median & 4 & \textbf{0.0093799} & 22.1641 & 0.84181 & 32.7756 & 0.085995 & 56.3389 & 0.012 & \textbf{17.0921} \\  
 & 8 & \textbf{0.015772} & 29.7582 & -- & -- & 0.098455 & 48.9718 & 0.020032 & \textbf{20.9878} \\                
\hline                                                                                                            
 & 2 & 0.0097589 & 21.3831 & -- & -- & 0.086257 & 57.7462 & \textbf{0.0081187} & \textbf{16.9658} \\              
Mean & 4 & 0.065282 & 25.912 & 0.88777 & 33.2528 & 0.094529 & 59.4144 & \textbf{0.012814} & \textbf{18.9145} \\   
 & 8 & 21.6667 & 43.0989 & -- & -- & 0.10426 & 51.0538 & \textbf{0.022802} & \textbf{23.7053} \\                  
\hline                                                                                                            
\end{tabular}                                                                                                     
\caption{\textcolor{red}{Quantitative Comparison between other sota methods and our on DiliGenT data on Joyful Yell scale.}}                             
\label{table:tab:diligent_comparison_sfs}                                                                         
\end{table*}                                                                                                      


==> tables/table_diligent_ups.tex <==
\begin{table*}                                                                                                     
\centering                                                                                                         
\begin{tabular}{|c|c|c|c|c|c|c|c|}                                                                                 
\hline                                                                                                             
3D-shape & SF & \multicolumn{2}{c|}{Image Based depth SR}  & \multicolumn{2}{c|}{\cite{Favaro2012}}  & \multicolumn{2}{c|}{Ours}  \\                                        
\hline                                                                                                             
 &  & RMSE & MAE & RMSE & MAE & RMSE & MAE \\                                                                      
\hline\hline                                                                                                             
 & 2 & 0.0077882 & 22.0061 & 0.027303 & 9.3907 & \textbf{0.0075916} & \textbf{7.4463} \\                           
bear & 4 & \textbf{0.0077919} & 18.9459 & 0.028366 & 11.1408 & 0.0086321 & \textbf{7.3654} \\                      
 & 8 & -- & -- & 0.041598 & 14.876 & \textbf{0.013424} & \textbf{7.0751} \\                                        
\hline                                                                                                             
 & 2 & 0.0077863 & 27.3694 & 0.045529 & 22.0961 & \textbf{0.0066561} & \textbf{12.8437} \\                         
buddha & 4 & 0.0078303 & 26.0488 & 0.052984 & 24.9351 & \textbf{0.0077721} & \textbf{13.0456} \\                   
 & 8 & -- & -- & 8.8151 & 86.7154 & \textbf{0.013443} & \textbf{14.2232} \\                                        
\hline                                                                                                             
 & 2 & \textbf{0.0078205} & 21.8645 & 0.04162 & 11.4011 & 0.0080221 & \textbf{6.1107} \\                           
cat & 4 & \textbf{0.0076492} & 19.0099 & 0.036211 & 12.0019 & 0.010465 & \textbf{6.5624} \\                        
 & 8 & -- & -- & 0.028969 & 14.4399 & \textbf{0.015428} & \textbf{7.3881} \\                                       
\hline                                                                                                             
 & 2 & 0.0078497 & 23.5131 & 0.028649 & 17.8906 & \textbf{0.0056474} & \textbf{11.7435} \\                         
cow & 4 & \textbf{0.007844} & 20.242 & 0.026979 & 18.7526 & 0.0084471 & \textbf{12.4157} \\                        
 & 8 & -- & -- & 0.022574 & 21.6708 & \textbf{0.015269} & \textbf{13.7085} \\                                      
\hline                                                                                                             
 & 2 & \textbf{0.0078938} & 27.6963 & 0.12798 & 72.9195 & 0.010806 & \textbf{11.6856} \\                           
goblet & 4 & \textbf{0.0078725} & 25.5665 & 0.14059 & 19.972 & 0.015592 & \textbf{12.3094} \\                      
 & 8 & -- & -- & 7.3205 & 69.1478 & \textbf{0.030855} & \textbf{14.2188} \\                                        
\hline                                                                                                             
 & 2 & \textbf{0.0078757} & \textbf{26.905} & 0.07492 & 32.7727 & 0.022718 & 30.793 \\                             
harvest & 4 & \textbf{0.0078363} & \textbf{25.2992} & 0.086368 & 37.802 & 0.029105 & 32.0317 \\                    
 & 8 & -- & -- & 8.8242 & 91.5084 & \textbf{0.04051} & \textbf{33.7185} \\                                         
\hline                                                                                                             
 & 2 & 0.0078648 & 23.3253 & 0.021591 & 11.4882 & \textbf{0.0064584} & \textbf{7.3597} \\                          
pot1 & 4 & \textbf{0.0078397} & 21.414 & 0.022727 & 11.9276 & 0.008057 & \textbf{7.511} \\                         
 & 8 & -- & -- & 0.024294 & 13.6306 & \textbf{0.014456} & \textbf{7.9025} \\                                       
\hline                                                                                                             
 & 2 & 0.0077881 & 24.092 & 0.024355 & 16.2553 & \textbf{0.0047215} & \textbf{9.3834} \\                           
pot2 & 4 & 0.0080123 & 22.2491 & 0.014828 & 16.4617 & \textbf{0.0066036} & \textbf{9.604} \\                       
 & 8 & -- & -- & 0.045677 & 20.8716 & \textbf{0.012599} & \textbf{10.0728} \\                                      
\hline                                                                                                             
 & 2 & \textbf{0.0077277} & 26.2419 & 0.076375 & 26.0778 & 0.010298 & \textbf{18.9261} \\                          
reading & 4 & \textbf{0.0076277} & 23.9732 & 8.8244 & 91.2695 & 0.015207 & \textbf{21.657} \\                      
& 8 & -- & -- & 8.8025 & 90.3114 & \textbf{0.028178} & \textbf{25.2537} \\                                        
\hline                                                                                                             
\hline                                                                                                             
 & 2 & 0.0078205 & 24.092 & 0.04162 & 17.8906 & \textbf{0.0075916} & \textbf{11.6856} \\                           
Median & 4 & \textbf{0.0078363} & 22.2491 & 0.036211 & 18.7526 & 0.0086321 & \textbf{12.3094} \\                   
 & 8 & -- & -- & 0.045677 & 21.6708 & \textbf{0.015269} & \textbf{13.7085} \\                                      
\hline                                                                                                             
 & 2 & \textbf{0.0078216} & 24.7793 & 0.052036 & 24.4769 & 0.0092132 & \textbf{12.9213} \\                         
Mean & 4 & \textbf{0.0078115} & 22.5276 & 1.0259 & 27.1404 & 0.012209 & \textbf{13.6114} \\                        
 & 8 & -- & -- & 3.7695 & 47.0191 & \textbf{0.020463} & \textbf{14.8401} \\                                        
\hline                                                                                                             
\end{tabular}                                                                                                      
\caption{\textcolor{red}{Quantitative Comparison between other sota methods and our ups approach on DiliGenT data}}
\label{table:tab:diligent_comparison_ups}                                                                          
\end{table*}                                                                                                       

